Firmware Insider: Bluetooth Randomness is Mostly Random

Bluetooth chips must include a Random Number Generator (RNG). This RNG is used internally within cryptographic primitives but also exposed to the operating system for chip-external applications. In general, it is a black box with security-critical authentication and encryption mechanisms depending on it. In this paper, we evaluate the quality of RNGs in various Broadcom and Cypress Bluetooth chips. We find that the RNG implementation significantly changed over the last decade. Moreover, most devices implement an insecure Pseudo-Random Number Generator (PRNG) fallback. Multiple popular devices, such as the Samsung Galaxy S8 and its variants as well as an iPhone, rely on the weak fallback due to missing a Hardware Random Number Generator (HRNG). We statistically evaluate the output of various HRNGs in chips used by hundreds of millions of devices. While the Broadcom and Cypress HRNGs pass advanced tests, it remains indistinguishable for users if a Bluetooth chip implements a secure RNG without an extensive analysis as in this paper. We describe our measurement methods and publish our tools to enable further public testing.

==> sections/removed.tex <==


\begin{figure}[!b]

\center

	\begin{center}
	\begin{tikzpicture}[minimum height=0.55cm, scale=0.8, every node/.style={scale=0.8}, node distance=0.7cm]
	
	% Devices 
    \node[inner sep=0pt] (iphonea) at (5,0)
    {\includegraphics[height=1.5cm]{pics/nexus.pdf}}; 
    \node[inner sep=0pt] (nexusx) at (7,0)
    {\includegraphics[height=1.1cm]{pics/nexus5.png}};  
    \node[inner sep=0pt] (iphone) at (7,0)
    {\includegraphics[height=1.5cm]{pics/iphone.pdf}}; 
    \node[inner sep=0pt] (iphonex) at (7,0)
    {\includegraphics[height=1.2cm]{pics/iphone.jpg}};  

    
    % Device Labels
    \node[below=of iphone.south, anchor=south, yshift=0.3cm] (iphonetxt) {Device $B$};
    \node[below=of iphonea.south, anchor=south, yshift=0.3cm] (iphonetxt) {Device $A$};
    
    
    % Device Lines
    \draw[-,gray,dashed,thick] (5,-1.3) -- (5,-7);
    \draw[-,gray,dashed,thick] (7,-1.3) -- (7,-7);
    
    \node[align=left,right] at (1, -2) {$LK\_K_A=$\\ \hspace*{3em}$E_{21}(LK\_RAND_A,$ \\ \hspace*{5em}$BD\_ADDR_A)$}; 
    \node[align=left,right] at (7, -2) {$LK\_K_B=$\\ \hspace*{3em}$E_{21}(LK\_RAND_B,$ \\ \hspace*{5em}$BD\_ADDR_B)$}; 
    
    \node[align=left,right] at (1, -3) {$C_A=$\textcolor{darkred}{$LK\_RAND_A$}$\oplus K$}; 
    \node[align=left,right] at (7, -3) {$C_B=LK\_RAND_B \oplus K$}; 
    
    \path[->] (5.2,-3.5) edge node[sloped, anchor=center, above, text width=0.5cm,yshift=-0em] {$C_A$} (6.7,-3.5);
    \path[<-] (5.2,-4) edge node[sloped, anchor=center, above, text width=0.5cm,yshift=-0em] {$C_B$} (6.7,-4);
    
    
    \node[align=left,right] at (1, -4.5) {$LK\_RAND_B = C_B \oplus K$};
    \node[align=left,right] at (1, -5.5) {$LK\_K_B=$\\ \hspace*{3em}$E_{21}(LK\_RAND_B,$ \\ \hspace*{5em}$BD\_ADDR_B)$}; 
    \node[align=left,right] at (1, -6.5) {$K_{AB} = LK\_K_A \oplus LK\_K_B$};
    
    \node[align=left,right] at (7, -4.5) {$LK\_RAND_A = C_A \oplus K$};
    \node[align=left,right] at (7, -5.5) {$LK\_K_A=$\\ \hspace*{3em}$E_{21}(LK\_RAND_A,$ \\ \hspace*{5em}$BD\_ADDR_A)$}; 
    \node[align=left,right] at (7, -6.5) {$K_{BA} = LK\_K_B \oplus LK\_K_A$};  
    
	\end{tikzpicture}
	\end{center}
	
\caption{Combination key generation. The old link key $K$ is discarded after successful exchange of a new combination key $K_{AB}$~\cite[p. 958]{bt52}.}
\label{fig:combkey}
\end{figure}

\subsection{Link Key Extraction via Combination Key LMP Packets}
The key management of Classic Bluetooth is described in Section 2.H.3 of the specification~\cite[p. 954ff]{bt52}.
Section 2.H.6 lists all algorithms in detail, including how random numbers are used within them~\cite[p. 976ff]{bt52}.

Classic Bluetooth has various types of link keys. The key types explained in the following are relevant for the outlined attack.
During initialization, $K_{init}$ is used. This is immediately withdrawn after
creating the permanent link key, also called combination key, $K_{AB}$. $K_{AB}$ is shared between a device $A$ and another
device $B$ and stored on the host. $K_{AB}$ authenticates connections between $A$ and $B$. Encryption is separated
from authentication by deriving an encryption key $K_C$ for each session.

Bluetooth works offline and without pre-installed certificates. Thus, the trust concept is \ac{TOFU}. If no PIN entry and
no \ac{SSP} are present, a passive \ac{MITM} can intercept an initial pairing and derive the same keys. Note that
\ac{SSP} can prevent passive and active \ac{MITM} attacks by adding a \ac{ECDH} key exchange. Typically, devices prevent
active \ac{MITM} attacks using the \ac{SSP} numeric comparison. During numeric comparison, a 6-digit number is displayed
on both devices and the user needs to actively confirm that these numbers are identical.

In the following, we assume that the attacker was not present when $K_{AB}$ was established insecurely or that the attacker
could not intercept $K_{AB}$ due to \ac{SSP}. However, the \ac{LMP} allows to refresh the permanent link key with the same combination key
method as in the upgrade from $K_{init}$ to $K_{AB}$.
In contrast to the initial pairing, this happens in the background and the user is not required to confirm authenticity.
When the link key is changed, the encryption is paused and continued after completion~\cite[p. 637]{bt52}, meaning that a
passive \ac{MITM} can intercept all traffic.
The combination key procedure is depicted in \autoref{fig:combkey}. An attacker who intercepts $C_A$ and knows the random number $LK\_RAND_A$
can undo the $\oplus$ operation to infer the old link key $K$ and also calculate the new link key $K_{AB}$.
$C_A$ is sent within the \path{LMP_COMB_KEY} \ac{PDU}~\cite[p. 625]{bt52}.

Note that if the attacker has additional access to a plaintext-ciphertext pair of the previous or next link key, the attack is even
possible if the randomness can only be predicted to be in a small set, as each possible key can be checked against the plaintext-ciphertext pair.

According to the specification, the encryption key $K_C$ should be refreshed at least every \SI{23.3}{\hour}~\cite[p. 952]{bt52}.
One of the two options to refresh the encryption keys is to update the link key $K_{AB}$ as described above. 
\todo{fr: What are the other methods? How common is this method used to update the Key?}
Thus, even if the initial key exchange was secured by the \ac{TOFU} principle, a passive \ac{MITM}
that observes a plaintext \path{LMP_COMB_KEY} \ac{PDU} and knows the current \ac{RNG} state can
extract the previous and next permanent link key. This breaks the encryption and authentication of a Classic Bluetooth connection.

We want to emphasize that due to this dependency on good randomness, the key update, a mechanism designed to increase the security
of the Bluetooth connection, actually increases the risk of an attack, and unnecessarily so. Being able to recover the previous permanent
link key during a key update means that an attacker can use the key update to decrypt data which would have been inaccessible if no further
key update would have been performed. Using a \ac{KDF} on the previous permanent link key before using it to encrypt the randomness sent over
the communication channel would have prevented this attack, and the overhead of a single call to a \ac{KDF} should be negligible. Further, if 
the key update protocol would have used a known-plaintext secure encryption function (i.e., basically anything more sophisticated than a 
simple XOR-encryption) to encrypt the randomness, neither the previous nor the next permanent link key would have leaked to the attacker 
even if they can predict the output of the \ac{RNG} perfectly.

